Theoretical Behavior of XAI Methods in the Presence of Suppressor Variables

In recent years, the community of 'explainable artificial intelligence' (XAI) has created a vast body of methods to bridge a perceived gap between model 'complexity' and 'interpretability'. However, a concrete problem to be solved by XAI methods has not yet been formally stated. As a result, XAI methods are lacking theoretical and empirical evidence for the 'correctness' of their explanations, limiting their potential use for quality-control and transparency purposes. At the same time, Haufe et al. (2014) showed, using simple toy examples, that even standard interpretations of linear models can be highly misleading. Specifically, high importance may be attributed to so-called suppressor variables lacking any statistical relation to the prediction target. This behavior has been confirmed empirically for a large array of XAI methods in Wilming et al. (2022). Here, we go one step further by deriving analytical expressions for the behavior of a variety of popular XAI methods on a simple two-dimensional binary classification problem involving Gaussian class-conditional distributions. We show that the majority of the studied approaches will attribute non-zero importance to a non-class-related suppressor feature in the presence of correlated noise. This poses important limitations on the interpretations and conclusions that the outputs of these XAI methods can afford.

==> images/pixel_flipping_tikz.tex <==
\begin{tikzpicture}
\begin{axis}[
    axis lines = left,
    xlabel = \(c\),
    ylabel = {\(f(c)\)},
]
%Below the red parabola is defined
\addplot [
    domain=-1:1, 
    samples=100, 
    color=red,
]
{1/(sqrt(1 + (x * 0.8/(abs(x)*0.8)))) * 0.8 * (2 * x * abs(x) * 0.8 - 0.8)};
\addlegendentry{\(x^2 - 2x - 1\)}
%Here the blue parabola is defined
\addplot [
    domain=-1:1, 
    samples=100, 
    color=blue,
    ]
    {0.1*x^2 + 2*x + 1};
\addlegendentry{\(x^2 + 2x + 1\)}

\end{axis}
\end{tikzpicture}
